Make the most of what you have: Resource-efficient randomized algorithms for matrix computations

In recent years, randomized algorithms have established themselves as fundamental tools in computational linear algebra, with applications in scientific computing, machine learning, and quantum information science. Many randomized matrix algorithms proceed by first collecting information about a matrix and then processing that data to perform some computational task. This thesis addresses the following question: How can one design algorithms that use this information as efficiently as possible, reliably achieving the greatest possible speed and accuracy for a limited data budget? The first part of this thesis focuses on low-rank approximation for positive-semidefinite matrices. Here, the goal is to compute an accurate approximation to a matrix after accessing as few entries of the matrix as possible. This part of the thesis explores the randomly pivoted Cholesky (RPCholesky) algorithm for this task, which achieves a level of speed and reliability greater than other methods for the same problem. The second part of this thesis considers the task of estimating attributes of an implicit matrix accessible only by matrix-vector products. This thesis describes the leave-one-out approach to developing matrix attribute estimation algorithms and develops optimized trace, diagonal, and row-norm estimation algorithms. The third part of this thesis considers randomized algorithms for overdetermined linear least squares problems. Randomized algorithms for linear-least squares problems are asymptotically faster than any known deterministic algorithm, but recent work has raised questions about the accuracy of these methods in floating point arithmetic. This thesis shows these issues are resolvable by developing fast randomized least-squares problem achieving backward stability, the gold-standard stability guarantee for a numerical algorithm.

==> index_stuff.tex <==
\index{kernel method|seealso{Gaussian process!type of machine learning method}}
\index{Gaussian process!type of machine learning method|seealso{kernel method}}
\index{overdetermined least squares|see{least squares}}
\index{linear least squares|see{least squares}}
\index{Blendenpik@\textsf{Blendenpik}|seealso{sketch-and-precondition}}
\index{sketching matrix|seealso{subspace embedding}}
\index{subspace embedding|seealso{sketching matrix}}
\index{low-rank approximation!for positive semidefinite matrices|see{positive semidefinite low-rank approximation}}
\index{randomized SVD!with subspace iteration|see{randomized subspace iteration}}
\index{positive semidefinite low-rank approximation!Nystr\"om approximation|see{Nystr\"om approximation}}
\index{low-rank matrix|see{low-rank approximation}}
\index{access models for matrices!matvec model|see{matvec model}}
\index{access models for matrices!entry access model|see{entry access model}}
\index{positive definite kernel function|see{kernel function}}
\index{low-rank approximation!near-optimality|see{r,epsilon,p-approximation@$(r,\varepsilon,p)$-approximation}}
\index{Cholesky decomposition!with pivoting|see{pivoted partial Cholesky decomposition}}
\index{pivoted partial Cholesky decomposition!greedy pivoting|see{greedy pivoted Cholesky}}
\index{Cholesky decomposition!greedy pivoting|see{greedy pivoted Cholesky}}
\index{complete pivoting|see{greedy pivoted Cholesky}}
\index{diagonal pivoting|see{greedy pivoted Cholesky}}
\index{Nystr\"om approximation!column Nystr\"om approximation|see{column Nystr\"om approximation}}
\index{pivoted partial Cholesky decomposition|seealso{column Nystr\"om approximation}}
\index{column Nystr\"om approximation|seealso{pivoted partial Cholesky decomposition}}
\index{leverage scores!ridge|see{ridge leverage scores}}
\index{column Nystr\"om approximation!by uniform sampling|see{uniform sampling for column Nystr\"om approximation}}
\index{column Nystr\"om approximation!by diagonal-power sampling|see{diagonal-power sampling for column Nystr\"om approximation}}
\index{column projection approximation!by squared column-norm sampling|see{squared column-norm sampling for column projection approximation}}
\index{column-norm sampling|see{squared column-norm sampling for column projection approximation}}
\index{row-norm sampling|see{squared column-norm sampling for column projection approximation}}
\index{reproducing kernel|seealso{kernel function}}
\index{kernel function|seealso{reproducing kernel}}
\index{kernel method!for interpolation|see{kernel interpolation}}
\index{interpolation!by kernels|see{kernel interpolation}}
\index{covariance function|seealso{kernel function}}
\index{Gaussian process regression|seealso{kernel ridge regression}}
\index{kernel ridge regression|seealso{Gaussian process regression}}
\index{Gaussian process interpolation|seealso{kernel interpolation}}
\index{kernel interpolation|seealso{Gaussian process interpolation}}
\index{ridge regularization!for kernel methods|see{kernel ridge regression}}
\index{ridge regularization!for kernel methods|see{Gaussian process interpolation}}
\index{Nystr\"om preconditioning|see{column Nystr\"om preconditioning}}
\index{preconditioning!by column Nystr\"om approximation|see{column Nystr\"om preconditioning}}
\index{randomly pivoted Cholesky!as a preconditioner|see{column Nystr\"om preconditioning}}
\index{preconditioned conjugate gradient|see{conjugate gradient}}
\index{randomly pivoted Cholesky!accelerated version|see{accelerated randomly pivoted Cholesky}}
\index{kernel ridge regression!restricted|see{restricted kernel ridge regression}}
\index{restricted kernel ridge regression|seealso{sparse Gaussian process regression}}
\index{sparse Gaussian process regression|seealso{restricted kernel ridge regression}}
\index{Nystr\"om method for kernel machine learning|see{restricted kernel ridge regression}}
\index{kernel method!Nystr\"om method|see{restricted kernel ridge regression}}
\index{Gaussian process regression!sparse|see{sparse Gaussian process regression}}
\index{column subset selection problem|see{subset selection problem}}
\index{randomly pivoted Cholesky!in infinite dimensions|see{infinite-dimensional randomly pivoted Cholesky}}
\index{quadrature|see{kernel quadrature}}
\index{reproducing kernel Hilbert space!quadrature on|see{kernel quadrature}}
\index{projection approximation!column projection approximation|see{column projection approximation}}
\index{column projection approximation!representation as a matrix factorization|seealso{pivoted partial QR decomposition}}
\index{column projection approximation!representation as a matrix factorization|seealso{interpolative decomposition}}
\index{adaptive sampling|see{randomly pivoted QR@randomly pivoted \QR}}
\index{volume sampling|seealso{determinantal point process sampling}}
\index{Nystr\"om approximation!generalized|see{generalized Nystr\"om approximation}}
\index{pseudoskeletal approximation|see{\CURnoindex approximation}}
\index{cross approximation|see{\CURnoindex approximation}}

==> old/low_rank_plus_shift.tex <==
\iffull

\chapter{Low-rank-plus-shift linear systems and Nystr\"om preconditioning revisited} \label{ch:low-rank-plus-and-nystrom}

\ENE{Consider adding me!}

\subsection{Background: Preconditioned conjugate gradient}

Krylov subspace methods are methods for solving linear systems of equations 
%
\begin{equation*}
    \mat{A}\vec{x} = \vec{b}
\end{equation*}
%
and other linear algebra problems using repeated matrix--vector products (matvecs) with the matrix $\mat{A}$.
For solving linear systems with a \warn{positive definite} matrix $\mat{A}$, the generally accepted method of choice is \emph{(preconditioned) conjugate gradient}, which we will abbreviate (P)CG.

Let $\mat{A}$ be a positive definite matrix and let $\mat{P}$ be a positive definite preconditioner; the case $\mat{P} = \Id$ yields standard, unpreconditioned, CG.
PCG requires access to the matrix $\mat{A}$ and inverse-preconditioner $\mat{P}^{-1}$ via subroutines
%
\begin{align*}
    \texttt{apply} &: \vec{z} \mapsto \mat{A}\vec{z}, \\
    \texttt{precond} &: \vec{z} \mapsto \mat{P}^{-1}\vec{z}.
\end{align*}
%
We emphasize that the matrices $\mat{A}$ and $\mat{P}^{-1}$ need not be stored explicitly in memory.
PCG works with any subroutines \texttt{apply} and \texttt{precond} that compute the action of the matrices $\mat{A}$ and $\mat{P}^{-1}$ on a vector $\vec{z}$.
PCG uses these operations to produce a sequence of iterates $\vec{x}^{(0)},\vec{x}^{(1)},\vec{x}^{(2)},\ldots$ that converge to the solution to $\mat{A}\vec{x} = \vec{b}$, at least in exact arithmetic.
(Understanding Krylov methods in floating point arithmetic will be a principle concern of \cref{part:sketching}.)

Preconditioned CG is equivalent to unpreconditioned CG on the \warn{symmetrically preconditioned} linear system 
%
\begin{equation} \label{eq:sym-pre-pd-system}
    (\mat{P}^{-1/2}\mat{A}\mat{P}^{-1/2})(\mat{P}^{1/2} \vec{x}) = \mat{P}^{-1/2}\vec{b}.
\end{equation}
%
The rate of convergence of PCG governed by the condition number 
%
\begin{equation*}
    \kappa_{\mathrm{pre}} \coloneqq \cond(\mat{P}^{-1/2}\mat{A}\mat{P}^{-1/2}).
\end{equation*}
%
of the symmetrically preconditioned matrix.
The fact that PCG is able to solve symmetrically preconditioned system \cref{eq:sym-pre-pd-system} while only requiring matvecs with $\mat{P}^{-1}$ and not its square root is essential in many applications.

\ENE{Standard error bound}

\subsection{Low-rank preconditioning for psd matrices}

First, we discuss low-rank preconditioning for psd matrices in general.
Consider the regularized system of linear equations
%
\begin{equation*}
    (\mat{A} + \lambda \Id)\vec{x} = \vec{b},
\end{equation*}
%
where $\mat{A} \in \field^{n\times n}$ is a psd matrix, $\lambda \in \real_+$ is a positive regularization, and $\vec{b} \in \field^n$.
Suppose we have a rank-$k$ approximation $\Ahat = \mat{V}\mat{D}\mat{V}^*\approx \mat{A}$, represented as a compact eigendecomposition.
The matrix $\mat{V} \in \field^{n\times k}$ has orthonormal columns, and $\mat{D} \in \real_+^{k\times k}$ is a psd diagonal matrix.
Define the general \emph{psd low-rank preconditioner}
%
\begin{equation} \label{eq:psd-preconditioner-general}
    \mat{P} \coloneqq \mat{V}(\mat{D} + \hat{\lambda}_1 \Id)\mat{V}^* + \hat{\lambda}_2 (\Id - \mat{V}\mat{V}^*) \approx \mat{A} + \lambda \Id.
\end{equation}
%
This preconditioner is characterized by parameters $\hat{\lambda}_1,\hat{\lambda}_2 \in \real_+$.

The literature contains at least two perspections for how to choose the parameters $\hat{\lambda}_1$ and $\hat{\lambda}_2$.
The first, and seemingly more natural, choice is to select
%
\begin{equation} \label{eq:nystrom-parameter-1}
    \hat{\lambda}_1 \coloneqq \hat{\lambda}_2 \coloneqq \lambda.
\end{equation}
%
For this choice, we have $\mat{P} = \Ahat + \lambda \Id$.
Since $\Ahat \approx \mat{A}$, it is natural to precondition $\mat{A} + \lambda \Id$ by $\mat{P} = \Ahat + \lambda \Id$.

The second choice is slightly more difficult to motivate.
Here, we set
%
\begin{equation}  \label{eq:nystrom-parameter-2}
    \hat{\lambda}_1 \coloneqq \lambda \quad \text{and} \quad \hat{\lambda}_2 \coloneqq d_{kk} + \lambda.
\end{equation}
%
Recall, $d_{kk}$ is the smallest diagonal entry of $\mat{D}$.
Provided $d_{kk} > 0$, it is the smallest nonzero eigenvalue of $\Ahat$.
To motivate this choice, suppose we have access to a perfect low-rank approximation $\Ahat = \lowrank{\mat{A}}_k = \mat{V}\mat{D}\mat{V}^*$.
The full eigendecomposition of $\mat{A}$ can be written as
%
\begin{equation*}
    \mat{A} = \onebytwo{\mat{V}}{\mat{V}_\perp} \twobytwo{\mat{D}}{\mat{0}}{\mat{0}}{\mat{D}_\perp} \onebytwo{\mat{V}}{\mat{V}_\perp}^* = \mat{V}\mat{D}\mat{V}^* + \mat{V}_\perp^{\vphantom{*}}\mat{D}_\perp^{\vphantom{*}}\mat{V}_\perp^*.
\end{equation*}
%
The subdominant eigenvectors are $\mat{V}_\perp \in \field^{n\times (n-k)}$ and the subdominant eigenvalue matrix is $\mat{D}_\perp = \Diag(\lambda_i(\mat{A}) : i>k)\in \real_+^{(n-k)\times (n-k)}$.
Then for the general preconditioner \cref{eq:psd-preconditioner-general}, we have
%
\begin{equation*}
    \mat{P}^{-1/2} \mat{A} \mat{P}^{-1/2} = \mat{V} [(\mat{D} + \lambda \Id)(\mat{D} + \hat{\lambda}_1 \Id)^{-1}] \mat{V}^* + \mat{V}_\perp^{\vphantom{*}} [\hat{\lambda}_2^{-1}(\mat{D}_\perp^{\vphantom{*}} + \lambda \Id)] \mat{V}_\perp^*,
\end{equation*}
%
and its eigenvalues are 
%
\begin{equation*}
    \underbrace{\left\{ \frac{\lambda_i(\mat{A}) + \lambda}{\lambda_i(\mat{A}) + \hat{\lambda}_1} : i \le k \right\}}_{\text{dominant eigenvalues after preconditioning}} \cup \underbrace{\left\{ \frac{\lambda_i(\mat{A}) + \lambda}{\hat{\lambda}_2} : i > k \right\}}_{\text{subdominant eigenvalues after preconditioning}}.
\end{equation*}
%
Thus, with $\hat{\lambda}_1 = \lambda$, preconditioning sets the $k$ top eigenvalues to $1$.
The choice $\hat{\lambda}_2 = d_{kk} + \lambda = \lambda_k(\mat{A}) + \lambda$ in \cref{eq:nystrom-parameter-2} leads to a gracefully decay in the subdominant eigenvalues.
By contrast, the parameter setting \cref{eq:nystrom-parameter-1} can cause large spikes in subdominant eigenvalues if $\lambda_{k+1}(\mat{A}) \gg \lambda$.

\fi
